Measurement of the branching fraction and decay asymmetry of $\Lambda\to n\gamma$

The radiative hyperon decay $\Lambda\to n\gamma$ is studied using $(10087\pm44)\times 10^6$ $J/\psi$ events collected with the BESIII detector operating at BEPCII. The absolute branching fraction of the decay $\Lambda\to n\gamma$ is determined with a significance of 5.6$\sigma$ to be $[0.832\pm0.038(\rm stat.)\pm0.054(\rm syst.)]\times10^{-3}$, which lies significantly below the current PDG value. By analyzing the joint angular distribution of the decay products, the first determination of the decay asymmetry $\alpha_{\gamma}$ is reported with a value of $-0.16\pm0.10(\rm stat.)\pm0.05(\rm syst.)$.

==> Contents.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The radiative hyperon decay is a puzzle because of Hara's theorem~\cite{Hara1964} which states 
that the parity violating amplitude of the decay should vanish in the limit of $\rm SU(3)$ flavor symmetry.
It came as a great surprise when the first measurement indicated a large negative asymmetry 
in the $\Sigma^{+}\to p\gamma$ decay~\cite{Manz1980,Kobayashi1987777,Foucher1992,Timm1995}.
More radiative hyperon decays have been measured experimentally %~\cite{Biagi:1986vn,Noble:1992ya, Larson:1993ig,James:1990as,Teige:1989uk,E761:1993unn,KTeV:2000dsr}
and found non-vanishing decay asymmtries~\cite{James1990,Teige1989,Foucher1992akkk}.
These observations raised wide interests among theorists and 
many solutions of the problems in the context of various models are 
proposed~\cite{Vasanti1976uuu,Kogan1983sss,Gilman1979asas,Goldman1989,Scadron1983,Palle1987,Zenczykowski1991}
%However, one of these models could
%describe satisfactorily both the large negative asymmetry and the observed rate of the sigma decay.
but regarded as controversial. 
However, there is an important quantative difference between the results of the two contradictory ways
of treating Hara's theorem,
and the decay asymmetry of $\Lambda\to n\gamma$ should be negative 
in Hara's theorem satisfying~\cite{Gavela1981a,Zenczykowski2006a,Niu2021zhao}
or positive in Hara's theorem violating~\cite{Zenczykowski2002,Zenczykowski1994}. 
It is proposed in Ref.~\cite{Zenczykowski2020a} that the measurements of $\Lambda\to n\gamma$ decay asymmetry could resolve the encountered
ambiguities and answer the question of whether Hara's theorem is violated or not.
%It is proposed in Ref.~  that
%the 

There are three measurements of $\Lambda\to n\gamma$ based on two 
fixed target experiments~\cite{Biagi:1986vn,Noble1992,Larson1993a},
where the branching fraction~(BF) is obtained as the ratio $\mathcal{B}_{\Lambdagn}/\mathcal{B}_{\Lambdapizn}$.
The results from the two experiments show poor agreement differing by about $2\sigma$.
The decay asymmetry of $\Lambda\to n\gamma$ is not determined due to limited statistics in Ref.~\cite{Biagi:1986vn}, while the decay asymmetry is not measurable with unpolarized $\Lambda$ in Ref.~\cite{Noble1992,Larson1993a}.
Therefore, a sound experiment that measures both the BF and the decay asymmetry of $\Lambdagn$ is of paramount importance to test theoretical ideas, and hopefully, solve the issue of Hara's theorem. 


At BESIII, a complete measurement of $\Lambdagn$ decay utilizing the relatively large BF of $\jpsill$~\cite{Li2017haibo} is realized with a double-tag~(DT) technique~\cite{Baltrusaitis1986}. Events of $\jpsill$ are identified by reconstructing the pionic decay $\Lambdapipb$,  denoted as single-tag (ST). A DT signal event consists of a ST $\bar\Lambda$ candidate accompanied with a $\Lambdagn$ signal candidate. The absolute BF is given by
\begin{equation}
\label{eq:branching ftaction}
    \frac{\mathcal{B}_{\Lambdagn}}{\mathcal{B}_{\Lambda\to anything}} =  \frac{N_{DT}/\varepsilon_{DT}} {N_{ST}/\varepsilon_{ST}}, 
\end{equation}
where $N_{ST}~(N_{DT})$ and $\varepsilon_{ST}~(\varepsilon_{DT})$ are the ST~(DT) yields and the detection efficiencies, respectively. Here and throughout this letter, charge conjugate channels are implied unless otherwise stated.

The $\Lambda$ from $\jpsill$ is transversely polarized with a maximum magnitude reaching 25\%~\cite{BESIIIPolirization2019}, which allows for the extraction of decay asymmetry in $\Lambda$ decay. The decay asymmetry of $\Lambdagn$ can be inferred from the angular distribution of the daughter baryons~\cite{Faeldt2017}. More generally, the joint angular distributions of $J/\psi\to\bar{\Lambda}(\to \bar{p}\pi^{+})\Lambda(\to n\gamma)$ can be expressed as: 
\begin{small}
\begin{equation}
\label{joint_angular_eq}
\begin{aligned}
&\mathcal{W}\left(\xi ; \alpha_{\psi}, \Delta \Phi, \alpha_{\gamma}, \alpha_{+}\right) \\
&=1+\alpha_{\psi} \cos ^{2} \theta_{\Lambda}+\alpha_{\gamma} \alpha_{+}\left[\sin ^{2} \theta_{\Lambda}\left(n^{1}_{x} n^{2}_{x}-\alpha_{\psi} n^{1}_{y} n^{2}_{y}\right)\right. \\
&\left.+\left(\cos ^{2} \theta_{A}+\alpha_{\psi}\right) n^{1}_{z} n^{2}_{z}\right] \\
&+\alpha_{\gamma} \alpha_{+} \sqrt{1-\alpha_{\psi}^{2}} \cos (\Delta \Phi) \sin \theta_{\Lambda} \cos \theta_{\Lambda}\left(n^{1}_{x} n^{2}_{z}+n^{1}_{z} n^{2}_{x}\right) \\
&+\sqrt{1-\alpha_{\psi}^{2}} \sin (\Delta \Phi) \sin \theta_{\Lambda} \cos \theta_{\Lambda}\left(\alpha_{\gamma} n^{1}_{y}+\alpha_{+} n^{2}_{y}\right),
\end{aligned}
\end{equation}
\end{small}where the $\hat{\textbf{n}}^{1}$~( $\hat{\textbf{n}}^{2}$) is the unit vector in the direction of the neutron(anti-proton, denoted as $\bar p$) in the rest frame of $\Lambda$~($\bar\Lambda$). The components of $\hat{\textbf{n}}^{1}$ and $\hat{\textbf{n}}^{2}$ are expressed using a coordinate system as $(n_{x}^{1},n_{y}^{1},n_{z}^{1})$ and $(n_{x}^{2},n_{y}^{2},n_{z}^{2})$ , in which the $z$ axis of both $\Lambda$ and $\bar\Lambda$ rest frames is oriented along the $\Lambda$ momentum $\mathbf{p}_{\Lambda}$ at an angle $\theta_{\Lambda}$ with respect to the $e^-$ beam direction. The $y$ axis is perpendicular to the production plane and oriented along the vector $\mathbf{k}_{-} \times \mathbf{p}_{\Lambda}$, where $\mathbf{k}_{-}$ is the $e^{-}$ beam momentum in the $\jpsi$ rest system. The $\alpha_{\psi}$ and $\Delta \Phi$ denote the absolute ratio of two helicity amplitudes of $\jpsill$ and their relative phase, respectively. The $\alpha_{\gamma}$ and $\alpha_{+}$ are the decay asymmetries for the $\Lambdagn$ and $\Lambdapipb$ decays, respectively. For each event, the full set of the kinematic variables~($\theta_{\Lambda}, \hat{\textbf{n}}_{1}, \hat{\textbf{n}}_{2}$) are denoted by the variable $\xi$.

In this letter, we report the absolute $\mathcal{B}_{\Lambda\to n\gamma}$ and the decay asymmetry $\alpha_{\gamma}$ of $\Lambda\to n\gamma$
 with $(10087\pm44)\times 10^6$ $\jpsi$ events~\cite{jpsinumber2021} collected at BESIII detector~\cite{Ablikim2010,Ablikim2020lalal} operating at the BEPCII~\cite{Yu2016}.% Precision of $\mathcal{B}_{\Lambda\to n\gamma}$ is improved and a discrepancy from world average value~\cite{Zyla2020} is observed.  The decay asymmetry $\alpha_{\gamma}$ is determined for the first time. 
Moverover, two independent $CP$ violating observables are constructed using the BF and $\alpha_{\gamma}$ measurement results from $\Lambdagn$ and its charge conjugate mode $\Lambdagnb$.\\

Simulated data samples produced with a {\sc Geant4}-based~\cite{G42002iii} Monte Carlo~(MC) package, which includes the detail geometric description of the BESIII detector and the detector response, are used to determine detection efficiencies and estimate backgrounds. The $\jpsi$ resonance is generated by the generator {\sc kkmc}~\cite{Jadach2001}, including the effects of the beam energy spread and the initial state radiation (ISR) in the $e^+e^-$ annihilation. The subsequent decays are modelled with {\sc EvtGen}~\cite{Lange2001} by incorporating the BFs taken from the PDG~\cite{Zyla2020}, and the remaining unknown decays are generated using {\sc LundCharm}~\cite{Chen2000}. %The final state radiations(FSR) from charged final state particles are incorporated with the $\sc{PHOTOS}$ package\cite{Barberio1994}. 
A sample of simulated events of $\jpsi$ decay~(denoted as inclusive MC sample) corresponding to the luminosity of data, is used to study backgrounds. Signal MC samples, including a sample of $5.6\times10^{7}$ $\jpsi\to\bar\Lambda~(\to \bar{p}\pi^{+})\Lambda~(\to\rm anything)$ and a sample of $4\times10^{5}$ $\jpsi\to\bar\Lambda~(\to \bar{p}\pi^{+})\Lambda~(\to n\gamma)$, are generated for signal efficiency estimation of ST and DT. Moreover, a sample of $2\times10^{7}$ $\jpsi\to\bar\Lambda~(\to \bar{p}\pi^{+})\Lambda~(\to n\pi^0)$ is generated to study the dominant background. The joint angular distributions in the generator model of the MC samples are formed according to Eq.~(\ref{joint_angular_eq}), with $\alpha_{\gamma}$ adopted from this analysis and other parameters from Ref.~\cite{BESIIIPolirization2019}. 

The ST $\bar\Lambda$ candidates are reconstructed through $\Lambdapipb$. Good charged tracks detected in the main drift chamber~(MDC) must satisfy $|\cos\theta|<0.93$, where $\theta$ is the polar angle with respect to the $z$-axis of the MDC. The pions and protons from $\bar\Lambda$ decays are well kinematically separated by momenta, thus the charged tracks with momenta less than 0.5~$\gevc$ are assigned to be pions, and those larger than 0.5~$\gevc$ are assigned to be protons. In addition, measurements of the specific ionization energy loss in the MDC and the time-of-flight are combined and used for particle identification by forming confidence levels~(CL) for particle hypothesis $i~(i=\pi/K/p)$, where proton candidates are required have the largest CL. Events with at least one $\bar p$ and one $\pi^{+}$ are selected. The $\bar p\pi^{+}$ combinations are constrained in a vertex fit and the one with minium $\chi_{\rm vtx}^{2}$ from the fit is selected. The $\chi_{\rm vtx}^{2}$ is further required to be less than 20. Moreover, the $\bar p \pi^{+}$ combination is required to have an invariant mass within 8~$\mevcc$ of the nominal $\Lambda$ mass~\cite{Zyla2020} and have the decay length of the reconstrcuted $\Lambda$ larger than two times of the its resolution. 

The contamination rate of the combinatorial background, estimated from the inclusive MC sample, is less than 1\%. The recoil mass of ST $\bar\Lambda$, $M^{\rm rec}_{\bar\Lambda} = \sqrt{ (E_{\rm beam} - E_{\bar\Lambda})^{2} - P_{\bar\Lambda}^{2}}$, is used to extract the ST yield, where $E_{\rm beam}$ is the beam energy, $E_{\bar\Lambda}$ and $P_{\bar\Lambda}$ are the energy and the momentum of ST $\bar\Lambda$ cadidate. A maximum likelihood fit to the spectrum of $M^{\rm rec}_{\bar\Lambda}$ is performed and the result is shown in Fig.~\ref{fig_ST_fit}, where the signal is represented by the MC shape convolved with a Gaussian function to account for imperfect simulation of the detector resolution, and the combinatorial backgrounds are described by a second order Chebyshev polynomial function. The ST yields are summarized in Table~\ref{tab:fit_results}. 
\begin{figure}[htbp]
\subfigure
{
  \begin{overpic}
    [scale=0.35]{Figures/singletag_fit_yield_n}\put(75,60){}
  \end{overpic}
}
	\caption{Distributions of $M^{\rm rec}_{\bar\Lambda}$ after ST
	selection. The black dots with error bars represent data, the red solid line shows the fit result and the blue dashed and green dotted lines are the distributions of signal and the background shapes, respectively.
}
\label{fig_ST_fit}
\end{figure}

The DT $\Lambda$ candidates are reconstructed through the $\Lambdagn$ with the residual neutral tracks in the presence of the ST $\bar\Lambda$ . For a good neutral shower, the deposited energy in the electromagnetic calorimeter~(EMC) should be larger than 25~MeV in the barrel region ($|\cos\theta| < 0.80$)
and larger than 50~MeV in the end cap region ($0.86<|\cos\theta|<0.92$).
To reject bremsstrahlung photons, showers matching the initial momentum of charged tracks within $10^{\circ}$ are discarded~($20^{\circ}$ for $\bar p$). To suppress electronic noise unrelated to events, the interval of the EMC response time and the event start time is required to be within 700~ns. In $\Lambdagn$, neutron~($n$) detection is not done due to its low detection efficiency and events are required to have at least one shower as photon candidate. A one-constraint~(1C) kinematic fit imposing energy-momentum conservation under the hypothesis $\jpsi\to\bar\Lambda n\gamma$ is implemented, wherein the $n$ is set as a missing particle. In $\Lambdagnb$, the most energetic shower with an over 400~MeV deposited energy is regarded as an anti-neutron~($\bar n$) candidate and events are required to have at least two showers as photon and $\bar n$ candidates. A three-constraint~(3C) kinematic fit that includes the $\bar{n}$ direction is performed under the hypothesis $\jpsi\to\Lambda \bar n\gamma$, wherein the energy of $\bar{n}$ is left as a free parameter. For events with more than one photon shower, all possible combinations are considered and the one giving the minimal $\chi_{1C}^2$ or $\chi_{3C}^2$ is selected , and $\chi_{1C}^2$ and $\chi_{3C}^2$ are further required to be less than 10 and 15, respectively.

One of the most challenges in this analysis is the photon detection for $\Lambdagn$ with the presence of a huge $\Lambdapizn$ background, which can be classified into two specific types: events with a photon candidate originating directly from $\pi^0$ decay~(BKGA); events with a photon candidate which is a noise shower from secondary products of other particles or other EMC noise~(BKGB). The other backgrounds except $\Lambdapizn$ are from $\Lambdapip$ and can be neglected. In order to suppress the BKGA, we apply a 1C~(3C) kinematic fit under the hypothesis $\jpsi\to\bar\Lambda n\gamma\gamma$~($\jpsi\to\Lambda \bar{n}\gamma\gamma$), and events passing the fit with an invariant mass of $\gamma\gamma$ pair~($M_{\gamma\gamma}$) within 20~$\mevcc$ of the nominal $\piz$ mass~\cite{Zyla2020} are rejected. After applying the above criteria, we find BKGB is dominant and will overlap with the signal in $E_{\gamma}^{\rm cms}$ distribution, as shown in Fig.~\ref{fig_DT_fit}. To further suppress the BKGB, two criteria are imposed on the kimematic properties of the selected photon: (1)~the energy of the selected photon is larger than 150~MeV, (2)~the openning angle between the selected photon and the neutron, $\sphericalangle_{n(\bar{n})}^{\gamma}$, is larger than 20$^\circ$. Additionally, a boosted decision tree~(BDT) is applied to discriminate signal photon from the noise showers, based on information of the $deposited$ $energy$, $secondary$ $moment$, $hit$ $number$, $Zernike$ $moment~(A_{42})$ and $deposition$ $ shape$~\cite{Zernikemoment}. We require the response of the BDT output to be larger than 0.3. After applying all above criteria, 86.8$\%$(92.8$\%$) of the BKGA and 99.5$\%$~(99.7$\%$) of the BKGB events are rejected for $\Lambdagn~(\Lambdagnb)$ process.  

To determine the DT signal yield, an unbinned extended maximum likelihood fit  is performed to the $E_{\gamma}^{\rm cms}$ distribution, as shown in Fig.~\ref{fig_DT_fit}. The signal and BKGA are modeled by the MC shape convolved with a Gaussian function. Since BKGB involves a noise photon and  cannot be well described by MC samples, we obtain the BKGB shape from data by control sample of $\Lambdapizn$, wherein the photon candidates used in kinematic fit are noise photons rather than the signal photons. The DT yields are summarized in Table~\ref{tab:fit_results}. The branching fractions are determined according to Eq.~(\ref{eq:branching ftaction}). It is found that the $\mathcal{B}_{\Lambdagn}$ is consistent with that of $\mathcal{B}_{\Lambdagnb}$ with uncertainties.
A simulatenous fit, assuming the same BF among the charge-conjugate modes, is performed and the BF is determined to be $[0.846\pm0.039(\rm stat.)]\times10^{-3}$.

The systematic uncertainties on the BF include the detection of photon and anti-neutron, kinematic fit, further requirements of $M_{\gamma\gamma}$ mass window and $\sphericalangle_{n(\bar{n})}^{\gamma}$, the MC model due to $\alpha_{\gamma}$ and the fit procedure.  The uncertainties for ST selection are canceled based on Eq.~(\ref{eq:branching ftaction}). The uncertainty associated with photon detection is $1\%$~\cite{Ablikimphoton2011}. The uncertainty of the anti-neutron detection efficiency is negligible after correcting the efficiency by a data-driven method~\cite{LiuLiang2021}. To estimate the uncertainty from the kinematic fit, the cut values of the $\chi^2_{1C}~(\chi^2_{3C})$ are varied and the largest difference of the BF with respect to the nominal result is taken as the uncertainty~($2.0\%$ for $\chi^2_{1C}$ and $1.5\%$ for $\chi^2_{3C}$ ).  The uncertainty from the requirement of $M(\gamma\gamma)$ mass window, is studied with the control sample of $\jpsi\to\bar\Lambda~(\to \bar{p}\pi^{+})\Lambda~(\to n\pi^0)\piz~(\to\gamma\gamma)$, and the difference between the data and MC efficiencies is taken as the  uncertainty~($1.2\%$). The uncertainty from the $\sphericalangle_{n(\bar{n})}^{\gamma}$ requirement is estimated to be $2.0\%$ by varying the criteria. The uncertainty associated with the BDT is negligible after correction of the efficiency using the control sample of $\jpsi\to\rho\pi~(\to\pi^{+}\pi^{-}\gamma\gamma)$ process. The uncertainty of signal efficiency due to the input decay asymmetry  $\alpha_{\gamma}$ in the MC generator is estimated to be $0.6\%$ by varying the input value of $\alpha_{\gamma}$ within its uncertainty. The systematic uncertainties from the fit procedure include the fit range and the modeling of the signal shape and background shapes. An alternative fit range for $E^{\rm cms}_{\gamma}$ of $(0.09, 0,23)$~GeV is used and the difference of the BF result to the nominal value is taken as the uncertainty~($0.3\%$). The uncertainties of the shape modeling of signal and BKGA, are estimated by varying the width of the convolved Gaussian function within uncertainties and the resultant differences of the fit results are taken as the systematic uncertainties~($0.4\%$ for signal and $1.0\%$ for BKGA). 
To estimate the shape modelling uncertainty of BKGB, 300 sets of toy-shapes are
generated based on the nominal BKGB shape and the resulting standard deviation of output BFs is taken as the systematic uncertainty~(4.8\%). The total systematic uncertainty is estimated to be $6.1\%$ by adding all these uncertainties in quadrature. 
\begin{table}[htbp]
\renewcommand\arraystretch{1.2}
\caption{The $ N_{ST}$, $\varepsilon_{ST}$, $N_{DT}$, $\varepsilon_{DT}$ for measuring $\Lambdagn$ and $\Lambdagnb$ process. The BF and $\alpha_{\gamma}$ are obtained from both individual fit and simultaneous fit. The fisrt uncertainties are statistical and the second uncertainties systematic.}
\label{tab:fit_results}
\centering
\scalebox{1.0}
{
\begin{tabular}{l c c}
\hline \hline 
\noalign{\vskip 3pt}
Decay Mode   & ~~~~~~$\Lambdagn$~~~~~~ & ~~~~~$\Lambdagnb$~~~~~ \\
\hline
$N_{ST}$ &  6736380$\pm$2750    &   6922930$\pm$2788  \\
$\varepsilon_{ST}~(\%)$&  51.13$\pm$0.01  & 52.53$\pm$0.01  \\
$N_{DT}$   & 498$\pm$41  & 723$\pm$40  \\
$\varepsilon_{DT}~(\%)$  &  4.20$\pm$0.03  & 6.59$\pm$0.04 \\ 
\hline
\multirow{2}{*}{$\mathcal{B}$~($\times10^{-3}$ )}  &~~~0.834$\pm$0.046$\pm$0.064~~~ & 0.876$\pm$0.071$\pm$0.082~~~ \\
     &  \multicolumn{2}{c}{\textbf{0.846$\pm$0.039$\pm$0.052}} \\
\hline
\multirow{2}{*}{$\alpha_{\gamma}$} & -0.13$\pm$0.13$\pm$0.02  &   0.21$\pm$0.15$\pm$0.06  \\
     &  \multicolumn{2}{c}{\textbf{-0.16$\pm$0.10$\pm$0.05}} \\
\hline
\hline
\end{tabular}
}
\end{table}


	\begin{figure}[htbp]
	\begin{center}
\begin{tikzpicture}[scale=1.0]
 \node(a) at (-1.0,0.0)
  {\includegraphics[width=1.0\linewidth]{Figures/simutaneouslyfit.pdf}\put(-220,72){\textbf{(a)}}\put(-96,72){\textbf{(b)}}}; 
\node(b) at (-2.0,-0.43)
  {\includegraphics[width=0.15\linewidth]{Figures/simutaneouslyfit_n.pdf}};
\node(c) at (2.33,-0.43)
  {\includegraphics[width=0.15\linewidth]{Figures/simutaneouslyfit_nbar.pdf}};
\end{tikzpicture}  
	\caption{Distributions of $E_{\gamma}^{\rm cms}$ for (a)$\Lambdagn$ and (b)$\Lambdagnb$ after all selection criteria. The solid, dashed, dotted and dashdotted lines denote the fit result, signal, BKGA and BKGB contributions. Histograms indicate the remaining BKGB from inclusive MC sample. The insets show the details of the fit in the signal region.  
}
\label{fig_DT_fit}
	\end{center}
	\end{figure}

The decay asymmetry $\alpha_{\gamma}$ is determined according to Eq.~(\ref{joint_angular_eq}), where an unbinned maximum likelihood fit is applied to the joint angular distribution $\mathcal{W}$ of the data after further requiring $E_{\gamma}^{\rm cms}$ within $(0.145, 0.17)$~GeV. 
In the fit, the likelihood function of $i_{th}$ event is constructed from the probability density function~(PDF):
\begin{equation}
\label{eql:pdf}
\begin{split} 
	 \mathcal{P}(\xi^{i}; \alpha_{\psi}, \Delta \Phi, \alpha_{\gamma}, \alpha_{+}) &= \mathcal{C}\mathcal{W}(\xi^{i}; \alpha_{\psi}, \Delta \Phi, \alpha_{\gamma}, \alpha_{+})\epsilon(\xi^{i}) , \\
\end{split} 
\end{equation}where $\mathcal{C}^{-1}= \int \mathcal{W}(\xi; \alpha_{\psi}, \Delta \Phi, \alpha_{\gamma}, \alpha_{+}) \epsilon(\xi)d\xi$ is the normalization factor evaluated by phase space~(PHSP) MC, and the $\alpha_{\psi}, \Delta \Phi, \alpha_{+}$ are fixed to values in Ref.~\cite{BESIIIPolirization2019}. The BKGA and BKGB contributions to the angular distribution are estimated with MC samples and subtracted when constructing the PDF. We perform individual fit for $\Lambdagn$ and $\Lambdagnb$ decay modes and the results are summarized in Table~\ref{tab:fit_results}. A simulatenous fit, assuming the same $\alpha_{\gamma}$ with opposite sign for the charge-conjugate modes, is adopted to determined the decay asymmetry to be $\alpha_{\gamma}(\Lambdagn)=-0.16\pm0.10(\rm stat.)\pm0.05(\rm syst.)$. The fit results are illustrated with the moment of $\cos\theta_{\Lambda}$ as shown in Fig~\ref{fig_moment_fit}. The moment is given by 
\begin{equation}
\label{eql:moment}
\begin{split} 
	 \mu(\cos\theta_{\Lambda}) & =  \frac{m}{N}\sum_{i=1}^{N_k}n_{y}^{1(2)}, \\
\end{split} 
\end{equation}which is calculated for $m=10$ bins in $\cos\theta_{\Lambda}$. $N$ is the total number of events in the data sample and $N_k$ is the number of events in the $k_{th} $ $\cos\theta_{\Lambda}$ bin. $n_{y}^{1}$~($n_{y}^{2}$) is the y components of unit vector in the direction of the $n$~($\bar p$) in the rest frame of $\Lambda$~($\bar\Lambda$). 

	\begin{figure}[htbp]
	\begin{center}
\begin{tikzpicture}[scale=1.0]
 \node(a) at (-1.0,0.0)
  {\includegraphics[width=1.0\linewidth]{Figures/Moment_deay_parameter_ngam.pdf}\put(-222,72){\textbf{(a)}}\put(-98,72){\textbf{(b)}}}; 
\end{tikzpicture}  
	\caption{Moment distributions $\mu(\cos\theta_{\Lambda}$) for (a)$\Lambdapipb$ and (b)$\Lambdagn$ in process $\jpsi\to\bar\Lambda~(\to \bar{p}\pi^{+})\Lambda~(\to n\gamma)$. For each event, the moment is calculated using Eq.~(\ref{eql:moment}) for $m=10$ bins in cos$\theta_{\Lambda}$. Dots with bars indicate data and solid lines show the result of the global fit based on Eq.~(\ref{eql:pdf}). The dashed and dotted lines represent moment distributions from signal MC and PHSP MC, respectively. }
\label{fig_moment_fit}
	\end{center}
	\end{figure}

The systematic uncertainties on the decay asymmetry $\alpha_{\gamma}$ come from similar sources as the BF except the detection of photon and anti-neutron, and the BDT requirements, which are considered of neglible effect to $\alpha_{\gamma}$. The uncertainties from kinematic fit are estimated by varying the cut value of the $\chi^2_{1C}~(\chi^2_{3C})$, and the maximum changes of $\alpha_{\gamma}$ to the nominal result is taken as the uncertainty~($0.024$ for $\chi^2_{1C}$ and $0.022$ for $\chi^2_{3C}$ ). The uncertainty due to the requirement of $M_{\gamma\gamma}$ mass widnow is estimated by varying the window from 20~$\mevcc$ to 27~$\mevcc$, yielding a difference of $\alpha_{\gamma}$ to the nominal result, to be 0.016, which is taken as the uncertainty. The uncertainty due to the requirement of $\sphericalangle_{n(\bar{n})}^{\gamma}$, is estimated to be 0.028 by taking the maximum changes of the $\alpha_{\gamma}$ to the nominal result when varying the corresponding cut value. The uncertainties due to fit range~(0.001), the signal modeling~(0.001), BKGA modeling~(0.002) and BKGB modeling~(0.008) are estimated using the same methods as the BF and the differences of $\alpha_{\gamma}$ to the nominal result are taken as the uncertainties. The total systematic uncertainty of $\alpha_{\gamma}$ is estimated to be 0.05 by adding all these uncertainties in quadrature. 

Two independent $CP$ violating observables $\Delta_{CP} = \frac{\mathcal{B}_{\Lambdagn}-\mathcal{B}_{\Lambdagnb}}{\mathcal{B}_{\Lambdagn}+\mathcal{B}_{\Lambdagnb}}$ and $A_{CP} = \frac{\mathcal{\alpha_{\gamma}}_{\Lambdagn}+\mathcal{\alpha_{\gamma}}_{\Lambdagnb}}{\mathcal{\alpha_{\gamma}}_{\Lambdagn}-\mathcal{\alpha_{\gamma}}_{\Lambdagnb}}$ are constructed with the individual results of BF and $\alpha_{\gamma}$ from the charge conjugate channels according to Ref.~\cite{He2001}. Finally, the $\Delta_{CP}$ and $A_{CP}$ are determined to be $-0.025\pm0.049(\rm stat.)\pm0.060(\rm syst.)$ and $-0.25\pm0.61(\rm stat.)\pm0.15(\rm syst.)$, which indicates that no $CP$ violation is observed under current statistics.  
%\begin{equation}
%\label{eql:cpodd_br}
%\begin{split} 
%	 \Delta_{CP} = \frac{\mathcal{B}(\Lambdagn)-\mathcal{B}(\Lambdagnb)}{\mathcal{B}(\Lambdagn)+\mathcal{B}(\Lambdagnb)} \\
%\end{split} 
%\end{equation}

%\begin{equation}
%\label{eql:cpodd_alpha}
%\begin{split} 
%	  A_{CP} = \frac{\mathcal{\alpha}(\Lambdagn)+\mathcal{\alpha}(\Lambdagnb)}{\mathcal{\alpha}(\Lambdagn)-\mathcal{\alpha}(\Lambdagnb)} \\
%\end{split} 
%\end{equation}

In summary, using $(10087\pm44)\times 10^6$ $\jpsi$ events collected with the BESIII detector, the radiative hyperon decay $\Lambdagn$ is studied at the electron-positron collider experiment for the first time. Based on the DT method, we report the first measurement of the absolute BF of $\Lambdagn$, to be $[0.846\pm0.039(\rm stat.)\pm0.052(\rm syst.)]\times10^{-3}$, which is smaller than world average value~$(1.75\pm0.15)\times10^{-3}$ by 5.4$\sigma$. By analyzing the joint angular distribution of the decay products, the decay asymmetry $\alpha_{\gamma}$ is determined for the first time, to be $-0.16\pm0.10(\rm stat.)\pm0.05(\rm syst.)$. The BF and $\alpha_{\gamma}$ are also measured individually for $\Lambdagn$ and $\Lambdagnb$ and the results are consistent within uncertainty. Two independent $CP$ violating observables are constructed for the two charge conjugate modes and no evidence of $CP$ violation is found. The negative $\alpha_{\gamma}$ indicates that Hara's theorem is still holds for radiative hyperon decay~\cite{Gavela1981a,Zenczykowski2006a,Niu2021zhao}. The smaller BF and almost vanishing $\alpha_{\gamma}$ measured in this analysis will provide essential input to constrain the amplitudes of parity violation contribution in theoretical calculations~\cite{Niu2021zhao,Vasanti1976uuu,Kogan1983sss,Gilman1979asas,Scadron1983,Palle1987,Zenczykowski1991}. 



